Flow: Per-Instance Personalized Federated Learning Through Dynamic Routing

Personalization in Federated Learning (FL) aims to modify a collaboratively trained global model according to each client. Current approaches to personalization in FL are at a coarse granularity, i.e. all the input instances of a client use the same personalized model. This ignores the fact that some instances are more accurately handled by the global model due to better generalizability. To address this challenge, this work proposes Flow, a fine-grained stateless personalized FL approach. Flow creates dynamic personalized models by learning a routing mechanism that determines whether an input instance prefers the local parameters or its global counterpart. Thus, Flow introduces per-instance routing in addition to leveraging per-client personalization to improve accuracies at each client. Further, Flow is stateless which makes it unnecessary for a client to retain its personalized state across FL rounds. This makes Flow practical for large-scale FL settings and friendly to newly joined clients. Evaluations on Stackoverflow, Reddit, and EMNIST datasets demonstrate the superiority in prediction accuracy of Flow over state-of-the-art non-personalized and only per-client personalized approaches to FL.

==> content/algo-simple.tex <==
\RestyleAlgo{ruled}
\begin{algorithm}[!h]
\footnotesize
\caption{Simplified version of \projectname{}}
\label{alg:flow-algo-simple}
\KwData{$R$: Total number of rounds,
$r \in [R]$: Round index,
$M$: Total number of clients,
$m \in [M]$: Client index,
$\cM{}$: Set of available clients,
$p$: Client sampling rate,
%$K$: Total local epoch count,
%$k \in [K]$: Epoch index,
$\eta_\ell$: Local learning rate,
$\wground{r}$: Global model at $r^{th}$ round,
$\wgclientround{r}$: $m^{th}$ client's local update of the global model for $r^{th}$ round,
$\wlround{r}$: $m^{th}$ client's local model for $r^{th}$ round,
$\wpround{r}$: $m^{th}$ client's personalized model for $r^{th}$ round,
$\psiground{r}$: Global policy model at $r^{th}$ round,
$\psigclientround{r}$: $m^{th}$ client's routing policy for $r^{th}$ round,
$\cD_{m}$: Data distribution of $m^{th}$ client 
} 
\KwResult{$\wground{R+1}$: Global model at the end of the training} 
Server randomly initializes $\wground{1}$ and $\psiground{1}$
\For{$r \in [R]$ round}{
    Sample $M$ clients from $\cM{}$ with the rate of $p$\\
    Send $\wground{r}$, $\psiground{r}$ to all the clients \\
    \For{$m \in [M]$ in parallel}{
        $\wgclientround{r} \gets w_{g}^{(r)}$;
        $\psigclientround{r} \gets \psiground{r}$;
        $\wlround{r} \gets \wgclientround{r} $\\
        $\datasetone{}, \datasettwo{} \gets \cD_{m}$ \Comment{Creating two mutually exclusive datasets}
        $\wlround{r+1} \gets \wlround{r} - \eta_\ell \nabla f_c (\wlround{r}; \datasetone{})$\\
        Define $\wpround{r}(x_m) \gets \psigclientround{r}(x_m) \cdot \wgclientround{r}(x_m) + (1 - \psigclientround{r}(x_m))\cdot \wlround{r+1}(x_m) \qquad \forall \; (x_m, y_m) \sim \datasettwo{} $\\ 
        $\psigclientround{r+1} \gets \psigclientround{r} - \eta_\ell \nabla_{\psigclientround{r}} \left[ f_c (\wpround{r}; \datasettwo{}) - \frac{\gamma}{N} \sum_{j\in [N]} \log(\psigclientround{r}[j])\right] $\\ 
        Define $\wpround{r}(x_m) \gets \psigclientround{r+1}(x_m) \cdot \wgclientround{r}(x_m) + (1 - \psigclientround{r+1}(x_m))\cdot \wlround{r+1}(x_m) \qquad \forall \; (x_m, y_m) \sim \datasettwo{} $\\ 
        $\wgclientround{r+1} \gets \wgclientround{r} - \ \eta_\ell \nabla_{\wgclientround{r}} f_c (\wpround{r}; \datasettwo{}) $\\ 
        Send back $\wgclientround{r+1}$, $\psigclientround{r+1}$, $n_m$ := $|\datasettwo{}|$
    }
    $\wground{r+1} \gets \frac{1}{nM} \sum_{m\in[M]} n_m \wgclientround{r} $\\ 
    $\psiground{r+1} \gets \frac{1}{nM} \sum_{m\in[M]} n_m \psigclientround{r}$
}
\end{algorithm}

==> dump.tex <==
% \begin{figure}[ht]
%     \captionsetup{justification=centering}
%     \centering
%     \begin{subfigure}{.32\linewidth}
%       \centering
%       \includegraphics[width=\linewidth]{diagrams/no_personalization.pdf}
%       \caption{No Personalization}
%       \label{fig:no-personalization}
%     \end{subfigure}
%     \begin{subfigure}{.32\linewidth}
%       \centering
%       \includegraphics[width=\linewidth]{diagrams/per_client_personalization_client_1.pdf}
%       \caption*{\phantom{}}
%     \end{subfigure}
%     \begin{subfigure}{.32\linewidth}
%       \centering
%       \includegraphics[width=\linewidth]{diagrams/per_instance_personalization_client_1.pdf}
%       \caption*{\phantom{}}
%     \end{subfigure}
    
%     % new row
%     \begin{subfigure}{.32\linewidth}
%       \centering
%       \includegraphics[width=\linewidth]{diagrams/per_instance_personalization.pdf}
%       \caption{Per-Instance\\Personalization}
%       \label{fig:per-instance-personalization}
%     \end{subfigure}
%     \begin{subfigure}{.32\linewidth}
%       \centering
%       \includegraphics[width=\linewidth]{diagrams/per_client_personalization_client_2.pdf}
%       \caption{Per-Client\\Personalization}
%       \label{fig:per-client-personalization}
%     \end{subfigure}
%     \begin{subfigure}{.32\linewidth}
%       \centering
%       \includegraphics[width=\linewidth]{diagrams/per_instance_personalization_client_2.pdf}
%       \caption{Per-Instance Per-Client Personalization (Proposed)}
%       \label{fig:per-instance-per-client-personalization}
%     \end{subfigure}
%     \captionsetup{justification=justified}
%     \caption{Illustration of different granularity of personalization using the computation graph of a machine learning model. Yellow and green nodes are model weights which are shared across clients. Edges represent tensors. Stripes and checks show different values of model parameters in two clients. Input-output pairs are colored in the same way as their activated execution path in a model.}
%     \label{fig:personalization-approaches}
% \end{figure}

% Figure~\ref{fig:personalization-approaches} illustrates the difference between per-client and per-instance personalization methods. 
% Without personalization (Figure \ref{fig:no-personalization}), all the clients and all the instances on a client execute the same model for prediction. 
% With only per-instance personalization (Figure~\ref{fig:per-instance-personalization}), all clients share the same global model but each input instance could activate a different part of the model for a prediction. 
% An issue with this granularity is that the same input on different clients would always produce the same output instead of a client-specific prediction.
% Per-client personalization (Figure \ref{fig:per-client-personalization}) has distinct personalized models for each client but all the instances on the same client use the same model. 
% Our proposed per-instance per-client personalization (Figure \ref{fig:per-instance-per-client-personalization}) allows instances on a client to flexibly choose which part of the personalized model to activate depending on a client-specific instance.

\begin{figure}[ht]
\begin{minipage}[b]{.33\textwidth}
    \centering
    \includegraphics[width=\textwidth]{plots/so_nwp_w_g_w_p_all_clients.pdf}
    \caption{Different combinations of $\wg{}$ and $\wper{}$ accuracies for Stackoverflow. Results for rest of the datasets are in Appendix \ref{adx:additional-results}, Figure \ref{fig:instance-stacked-bars}.}
    \label{fig:so-nwp-instance-stacked-bars}
\end{minipage}
\hfill
\begin{minipage}[b]{.66\textwidth}
\centering
    \begin{subfigure}[b]{0.49\textwidth}
         \centering
        \includegraphics[width=\textwidth]{plots/so_nwp_regularization_Flow.pdf}
         \caption{Ablation of the regularization term used in the policy learning objective for Stackoverflow. Results for rest of the datasets are in Appendix \ref{adx:additional-results}, Figure \ref{fig:regularization}.}
         \label{fig:so-nwp-regularization}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{plots/so_nwp_pcpi_Flow_variants.pdf}
         \caption{Ablation of the dynamic routing component (Per-client \projectname{}), and the local component (Per-instance \projectname{}). Results for rest of the datasets are in Appendix \ref{adx:additional-results}, Figure \ref{fig:ablation-pcpi}}
         \label{fig:so-nwp-ablation-pcpi}
     \end{subfigure}
    \caption{Ablation studies.}
    \label{fig:ablation}
\end{minipage}
\end{figure}
